Unbinned multivariate observables for global SMEFT analyses from machine learning

Theoretical interpretations of particle physics data, such as the determination of the Wilson coefficients of the Standard Model Effective Field Theory (SMEFT), often involve the inference of multiple parameters from a global dataset. Optimizing such interpretations requires the identification of observables that exhibit the highest possible sensitivity to the underlying theory parameters. In this work we develop a flexible open source framework, ML4EFT, enabling the integration of unbinned multivariate observables into global SMEFT fits. As compared to traditional measurements, such observables enhance the sensitivity to the theory parameters by preventing the information loss incurred when binning in a subset of final-state kinematic variables. Our strategy combines machine learning regression and classification techniques to parameterize high-dimensional likelihood ratios, using the Monte Carlo replica method to estimate and propagate methodological uncertainties. As a proof of concept we construct unbinned multivariate observables for top-quark pair and Higgs+$Z$ production at the LHC, demonstrate their impact on the SMEFT parameter space as compared to binned measurements, and study the improved constraints associated to multivariate inputs. Since the number of neural networks to be trained scales quadratically with the number of parameters and can be fully parallelized, the ML4EFT framework is well-suited to construct unbinned multivariate observables which depend on up to tens of EFT coefficients, as required in global fits.

==> flowchart.tex <==

\tikzstyle{startstop} = [rectangle, rounded corners, minimum width=3cm, minimum height=0.5cm,text centered, draw=black, fill=red!30]
\tikzstyle{io} = [trapezium, trapezium left angle=70, trapezium right angle=110, minimum width=3cm, minimum height=1cm, text centered, draw=black, fill=blue!30]
\tikzstyle{decision} = [diamond, minimum width=3cm, minimum height=1cm, text centered, draw=black, fill=green!30]
\tikzstyle{arrow} = [thick,->,>=stealth]
\tikzstyle{process} = [rectangle, minimum width=4cm, minimum height=1cm, text centered, draw=black, fill=orange!30, rounded corners, text width=4cm]

% \begin{tikzpicture}[node distance=2cm]
% \node (start) [startstop] {Start};
% \node (in1) [io, below of=start] {Input};
% \node (pro1) [process, below of=in1] {Process 1};
% \node (dec1) [decision, below of=pro1, yshift=-0.5cm] {Decision 1};
% \node (pro2a) [process, below of=dec1, yshift=-0.5cm] {Process 2a text text text text text text text text text text};
% \node (pro2b) [process, right of=dec1, xshift=2cm] {Process 2b};
% \node (out1) [io, below of=pro2a] {Output};
% \node (stop) [startstop, below of=out1] {Stop};
% \draw [arrow] (start) -- (in1);
% \draw [arrow] (in1) -- (pro1);
% \draw [arrow] (pro1) -- (dec1);
% \draw [arrow] (dec1) -- (pro2a);
% \draw [arrow] (dec1) -- (pro2b);

% \draw [arrow] (dec1) -- node[anchor=east] {yes} (pro2a);
% \draw [arrow] (dec1) -- node[anchor=south] {no} (pro2b);
% \draw [arrow] (pro2b) |- (pro1);
% \draw [arrow] (pro2a) -- (out1);
% \draw [arrow] (out1) -- (stop);
% \end{tikzpicture}
\begin{figure}[htbp]
\small
    \centering
    \begin{tikzpicture}[node distance=2cm]

\node (in1) [io] {\verb|smeftsim_main.fr|};
\node (pro1) [process, below of=in1] {\verb|SMEFTsim| \verb|Flavor = topU3l|, \verb|Scheme=MwScheme|};
\node (out1) [io, below left=of pro1] {\verb|FeynArts .mod file|};
\node (out2) [io, below right=of pro1] {\verb|FeynArts .gen file|};
\node (pro2a) [process, below of=pro1, node distance=6cm] {\verb|FeynArts|: draw topologies and insert fields};
\node (pro2b) [process, below of=pro2a] {\verb|FormCalc|: compute $\left|\mathcal{M}_{\mathrm{sm}} + \mathcal{M}_{\mathrm{eft}}(\boldsymbol{c})\right|^2$};
\node (pro2c) [process, below of=pro2b] {\verb|Mathematica|: compute $d\sigma(\boldsymbol{c})$};
\node (out3) [io, below of=pro2c] {Analytical $d\sigma(\boldsymbol{c})$};
% \node (out1) [io, below of=pro2a] {Output};
% \node (stop) [startstop, below of=out1] {Stop};

\draw [arrow] (in1) -- (pro1);
% \draw [arrow] (pro1) -- (dec1);
% \draw [arrow] (dec1) -- (pro2a);
% \draw [arrow] (dec1) -- (pro2b);

% \draw [arrow] (dec1) -- node[anchor=east] {yes} (pro2a);
% \draw [arrow] (dec1) -- node[anchor=south] {no} (pro2b);
\draw [arrow] (pro1) -| (out1);
\draw [arrow] (pro1) -| (out2);
\draw [arrow] (out1) |- (pro2a);
\draw [arrow] (out2) |- (pro2a);
\draw [arrow] (pro2a) -- (pro2b);
\draw [arrow] (pro2b) -- (pro2c);
\draw [arrow] (pro2c) -- (out3);
% \draw [arrow] (pro2a) -- (out1);
% \draw [arrow] (out1) -- (stop);
\end{tikzpicture}
    \caption{Flow diagram indicating the pipeline adopted
    in this work to evaluate analytical expressions
    of differential distributions in the SMEFT for
    the LHC processes considered.
    %
    These analytical cross-section are evaluated at leading order
    and at the parton level, where they are compared
    with numerical simulations
    for the same theoretical settings.
    %
    The analytical cross-section provide access to the
    exact likelihood ratio, which in turn makes possible a reference
    benchmark for the performance of the ML algorithm.
    }
    \label{fig:pipeline_flowchart}
\end{figure}


==> tables/datasets_tt_inclusive.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[htbp]
%\begin{table}[t]
  \centering
  \scriptsize
   \renewcommand{\arraystretch}{1.80}
  \begin{tabular}{c|c|c|c|c|c}
 Dataset   &  $\sqrt{s}$, $\mathcal{L}$  & Info  &  Observables  & $n_{\rm dat}$ & Ref   \\
    \toprule
      \multirow{2}{*}{ {\tt ATLAS\_tt\_8TeV\_ljets}}      &
    \multirow{2}{*}{{ \bf 8 TeV, 20.3~fb$^{-1}$}}   &  \multirow{2}{*}{lepton+jets}   & $
        d\sigma/d|y_{t}|$, $
        d\sigma/dp^T_{t}$,      & 5, 8,   & \multirow{2}{*}{\cite{Aad:2015mbv}}  \\
          &   &   & $
        d\sigma/dm_{t\bar{t}}$, $
        d\sigma/d|y_{t\bar{t}}|$      &  7, 5  &    \\
%-------------------------------------------------------------------------------
        \midrule
           \multirow{2}{*}{ {\tt CMS\_tt\_8TeV\_ljets}}      &
    \multirow{2}{*}{{\bf 8 TeV, 20.3~fb$^{-1}$}}   &  \multirow{2}{*}{lepton+jets}   & $
        d\sigma/dy_{t}$, $
        d\sigma/dp^T_{t}$,      &  10, 8,  &
        \multirow{2}{*}{\cite{Khachatryan:2015oqa}}  \\
          &   &   & $ 
        d\sigma/dm_{t\bar{t}}$, $
        d\sigma/dy_{t\bar{t}}$      & 7, 10 &    \\
%-------------------------------------------------------------------------------
        \midrule
      \multirow{4}{*}{ {\tt CMS\_tt2D\_8TeV\_dilep}}      &
\multirow{4}{*}{{\bf 8 TeV, 20.3~fb$^{-1}$}}   &  \multirow{4}{*}{dileptons}   &
$d^2\sigma/dy_{t}dp^T_{t}$,
             &  16,   &
        \multirow{4}{*}{\cite{Sirunyan:2017azo}}  \\
                   &   &   &  $d^2\sigma/dy_{t}dm_{t\bar{t}}$, & 16, &  \\
          &   &   & $d^2\sigma/dp^T_{t\bar{t}}dm_{t\bar{t}}$, & 16, 
        &    \\
                   &   &   &
        $d^2\sigma/dy_{t\bar{t}}dm_{t\bar{t}}$  & 16
        &    \\
%-------------------------------------------------------------------------------
        \midrule
      \multirow{2}{*}{ {\tt ATLAS\_tt\_8TeV\_dilep} {\bf(*)}}       &
\multirow{2}{*}{{\bf 8 TeV, 20.3~fb$^{-1}$}}   &  \multirow{2}{*}{dileptons}   &
 $d\sigma/dm_{t\bar{t}}$,$d\sigma/dp_{T,t\bar{t}}$ & 6,5 & \multirow{2}{*}{\cite{Aaboud:2016iot}}  \\
            &   &   & $d\sigma/d|y_{t\bar{t}}|$ & 5 &    \\
  %-------------------------------------------------------------------------------
\midrule
\midrule
      \multirow{2}{*}{ {\tt CMS\_tt\_13TeV\_ljets\_2015 }}      &
 \multirow{2}{*}{{\bf 13 TeV, 2.3~fb$^{-1}$}}   &  \multirow{2}{*}{lepton+jets}   & $
 d\sigma/d|y_{t}|$, $
  d\sigma/dp^T_{t},$      &  7, 9,  &
   \multirow{2}{*}{\cite{Khachatryan:2016mnb}}  \\
           &   &     &    $
 d\sigma/dm_{t\bar{t}}$, $
 d\sigma/d|y_{t\bar{t}}|$      &  8, 6   \\
 %-------------------------------------------------------------------------------
   \midrule
     \multirow{2}{*}{ {\tt CMS\_tt\_13TeV\_dilep\_2015 }}      &
 \multirow{2}{*}{{\bf 13 TeV, 2.1~fb$^{-1}$}}   &  \multirow{2}{*}{dileptons}   & $
  d\sigma/dy_{t}$, $
    d\sigma/dp^T_{t},$      &  8, 6,  &
   \multirow{2}{*}{\cite{Sirunyan:2017mzl}}  \\
           &   &     &    $
   d\sigma/dm_{t\bar{t}}$, $
   d\sigma/dy_{t\bar{t}}$      &  6, 8   \\
%-------------------------------------------------------------------------------
\midrule
      \multirow{2}{*}{ {\tt CMS\_tt\_13TeV\_ljets\_2016 }}      &
 \multirow{2}{*}{{\bf 13 TeV, 35.8~fb$^{-1}$}}   &  \multirow{2}{*}{lepton+jets}   & $
 d\sigma/d|y_{t}|$, $
  d\sigma/dp^T_{t},$      &  11, 12,  &
   \multirow{2}{*}{\cite{Sirunyan:2018wem}}  \\
          &   &     &    $
   d\sigma/dm_{t\bar{t}}$,
   $d\sigma/d|y_{t\bar{t}}|$      &  10, 10   \\
\midrule
      \multirow{2}{*}{ {\tt CMS\_tt\_13TeV\_dilep\_2016 } {\bf(*)}}      &
 \multirow{2}{*}{{\bf 13 TeV, 35.8~fb$^{-1}$}}   &  \multirow{2}{*}{dileptons}   & $
 d\sigma/d|y_{t}|$, $
  d\sigma/dp^T_{t},$      &  10, 6,  &
   \multirow{2}{*}{\cite{Sirunyan:2018ucr}}  \\
          &   &     &    $
   d\sigma/dm_{t\bar{t}}$,
   $d\sigma/d|y_{t\bar{t}}|$      &  7, 10   \\
 %-------------------------------------------------------------------------------
\midrule
         \multirow{2}{*}{ {\tt ATLAS\_tt\_13TeV\_ljets\_2016 } {\bf (*)}}      &
 \multirow{2}{*}{{\bf 13 TeV, 35.8~fb$^{-1}$}}   &  \multirow{2}{*}{lepton+jets}   & $
 d\sigma/d|y_{t}|$, $
  d\sigma/dp^T_{t},$      &  5, 8,  &
   \multirow{2}{*}{\cite{Aad:2019ntk}}  \\
          &   &     &    $
   d\sigma/dm_{t\bar{t}}$,
    $d\sigma/d|y_{t\bar{t}}|$      &  9, 7   \\
%-------------------------------------------------------------------------------
   \midrule
%-------------------------------------------------------------------------------

\bottomrule
  \end{tabular}
  \vspace*{5mm}
  \caption{{\bf Vero: I guess we need to add the same info but for HV in 2L}}
\label{eq:datasets_tt_inclusive}


\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> tables/fisher_tt_inclusive.tex <==
\begin{table}[htbp]
\footnotesize
\centering
\renewcommand{\arraystretch}{1.50}
\begin{tabular}{|c|c|c|c|}
\hline
 \multicolumn{2}{|c|}{} & \multicolumn{2}{c|}{Processes} \\ \hline
 Class & Coefficient & $t\bar{t}$ (8 TeV) & $t\bar{t}$ (13 TeV) \\ \hline
\multirow{14}{*}{2L2H}
 & {\color{blue}$c_{qq}^{1,8}$} & { \color{black} 1.003}({\color{black} -0.260}) & { \color{black} 2.710}({\color{black} 1.923})\\ \cline{2-4} 
 & $c_{qq}^{1,1}$ & { \color{black} 0.000}({\color{black} -4.743}) & { \color{black} 0.000}({\color{black} 7.211})\\ \cline{2-4} 
 & $c_{qq}^{8,3}$ & { \color{black} 0.086}({\color{black} -1.006}) & { \color{black} 0.157}({\color{black} 2.164})\\ \cline{2-4} 
 & $c_{qq}^{1,3}$ & { \color{black} 0.000}({\color{black} -4.788}) & { \color{black} 0.000}({\color{black} 7.384})\\ \cline{2-4} 
 & {\color{blue}$c_{qt}^{8}$} & { \color{black} 0.997}({\color{black} -0.294}) & { \color{black} 2.802}({\color{black} 2.185})\\ \cline{2-4} 
 & $c_{qt}^{1}$ & { \color{black} 0.000}({\color{black} -4.929}) & { \color{black} 0.000}({\color{black} 6.670})\\ \cline{2-4} 
 & {\color{blue}$c_{ut}^{8}$} & { \color{black} 0.414}({\color{black} -0.305}) & { \color{black} 1.097}({\color{black} 1.146})\\ \cline{2-4} 
 & $c_{ut}^{1}$ & { \color{black} 0.000}({\color{black} -3.229}) & { \color{black} 0.000}({\color{black} 4.280})\\ \cline{2-4} 
 & {\color{blue}$c_{qu}^{8}$} & { \color{black} 0.411}({\color{black} -0.321}) & { \color{black} 1.187}({\color{black} 1.174})\\ \cline{2-4} 
 & $c_{qu}^{1}$ & { \color{black} 0.000}({\color{black} -3.193}) & { \color{black} 0.000}({\color{black} 4.251})\\ \cline{2-4} 
 & {\color{blue}$c_{dt}^{8}$} & { \color{black} 0.132}({\color{black} -0.301}) & { \color{black} 0.353}({\color{black} 0.888})\\ \cline{2-4} 
 & $c_{dt}^{1}$ & { \color{black} 0.000}({\color{black} -1.753}) & { \color{black} 0.000}({\color{black} 2.328})\\ \cline{2-4} 
 & {\color{blue}$c_{qd}^{8}$} & { \color{black} 0.129}({\color{black} -0.313}) & { \color{black} 0.355}({\color{black} 0.901})\\ \cline{2-4} 
 & $c_{qd}^{1}$ & { \color{black} 0.000}({\color{black} -1.768}) & { \color{black} 0.000}({\color{black} 2.347})\\ \hline
\multirow{1}{*}{2FB}
 & {\color{blue}$c_{tG}$} & { \color{black} 96.829}({\color{black} 127.204}) & { \color{black} 91.339}({\color{black} 55.149})\\ \hline
\end{tabular}
\vspace*{5mm}
\caption{The normalised Fisher information for $t\bar{t}$ inclusive production at 8 TeV (left) and 13 TeV (right) grouped by operator class. We show results both at the linear level as well as the quadratic level in the EFT expansion, where the latter are given in parenthesis.}
\label{eq:fisher_tt_inclusive}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> tables/fisher_vh.tex <==
\begin{table}[H]
\footnotesize
\centering
\begin{tabular}{|c|c|c|}
\hline
 Class & Coefficient &  \href{https://arxiv.org/abs/1903.04618}{${\rm ATLAS\_ZH\_Hbb\_13TeV}$} \\ \hline
\multirow{14}{*}{2L2H}
 & $c_{qq}^{1,8}$ & { \color{black} 0.000}({\color{black} 0.000})\\ \cline{2-3} 
 & $c_{qq}^{1,1}$ & { \color{black} 0.000}({\color{black} 0.000})\\ \cline{2-3} 
 & $c_{qq}^{8,3}$ & { \color{black} 0.000}({\color{black} 0.000})\\ \cline{2-3}
 & $c_{qq}^{1,3}$ & { \color{black} 0.000}({\color{black} 0.000})\\ \cline{2-3} 
 & $c_{qt}^{8}$ &  { \color{black} 0.000}({\color{black} 0.000})\\ \cline{2-3}
 & $c_{qt}^{1}$ &  { \color{black} 0.000}({\color{black} 0.000})\\ \cline{2-3} 
 & $c_{ut}^{8}$ &  { \color{black} 0.000}({\color{black} 0.000})\\ \cline{2-3} 
 & $c_{ut}^{1}$ & { \color{black} 0.000}({\color{black} 0.000})\\ \cline{2-3} 
 & $c_{qu}^{8}$ & { \color{black} 0.000}({\color{black} 0.000})\\ \cline{2-3}
 & $c_{qu}^{1}$ &  { \color{black} 0.000}({\color{black} 0.000})\\ \cline{2-3}
 & $c_{dt}^{8}$ &  { \color{black} 0.000}({\color{black} 0.000})\\ \cline{2-3}
 & $c_{dt}^{1}$ &  { \color{black} 0.000}({\color{black} 0.000})\\ \cline{2-3}
 & $c_{qd}^{8}$ &  { \color{black} 0.000}({\color{black} 0.000})\\ \cline{2-3}
 & $c_{qd}^{1}$ & { \color{black} 0.000}({\color{black} 0.000})\\ \hline
\multirow{10}{*}{2FB}
 & $c_{t \varphi}$ &  { \color{black} 0.000}({\color{black} 0.000})\\ \cline{2-3}
 & $c_{tG}$ &  { \color{black} 0.000}({\color{black} 0.000})\\ \cline{2-3}
 & $c_{b \varphi}$ & { \color{blue} 0.000}({\color{blue} 0.000})\\ \cline{2-3}
 & $c_{c \varphi}$ &  { \color{black} 0.000}({\color{black} 0.000})\\ \cline{2-3}
 & $c_{\tau \varphi}$ & { \color{black} 0.000}({\color{black} 0.000})\\ \cline{2-3} 
 & $c_{tW}$ & { \color{black} 0.000}({\color{black} 0.000})\\ \cline{2-3}
 & $c_{tZ}$ &  { \color{black} 0.000}({\color{black} 0.000})\\ \cline{2-3}
 & $c_{\varphi Q}^{3}$ & { \color{black} 0.007}({\color{black} 1.980})\\\cline{2-3}
 & $c_{\varphi Q}^{(-)}$ & { \color{black} 0.002}({\color{black} 3.031})\\ \cline{2-3} 
 & $c_{\varphi t}$ &  { \color{black} 0.000}({\color{black} 0.000})\\ \hline
\multirow{6}{*}{B}
 & $c_{\varphi G}$ &{ \color{black} 0.000}({\color{black} 0.000})\\ \cline{2-3}
 & $c_{\varphi B}$ & { \color{blue} 0.006}({\color{blue} 0.001})\\ \cline{2-3}
 & $c_{\varphi W}$ &  { \color{blue} 0.423}({\color{blue} 16.162})\\ \cline{2-3} 
 & $c_{\varphi WB}$ &  { \color{blue} 84.717}({\color{blue} 25.306})\\ \cline{2-3}
 & $c_{\varphi d}$ & { \color{blue} 0.008}({\color{blue} 0.028})\\ \cline{2-3}
 & $c_{\varphi D}$ &{ \color{blue} 14.838}({\color{blue} 53.492})\\ \hline
\end{tabular}
	\caption{The normalised Fisher information for $ZH$ production, $Z\rightarrow \ell \ell$, $H \rightarrow b \bar{b}$ at 13 TeV grouped by operator class. We show results both at the linear level as well as the quadratic level in the EFT expansion, where the latter are given in parenthesis. {\color{red} update $c_{b\varphi}$}\label{tab:fisher_vh}}
\end{table}

